DiffMIC: Dual-Guidance Diffusion Network for Medical Image Classification

Diffusion Probabilistic Models have recently shown remarkable performance in generative image modeling, attracting significant attention in the computer vision community. However, while a substantial amount of diffusion-based research has focused on generative tasks, few studies have applied diffusion models to general medical image classification. In this paper, we propose the first diffusion-based model (named DiffMIC) to address general medical image classification by eliminating unexpected noise and perturbations in medical images and robustly capturing semantic representation. To achieve this goal, we devise a dual conditional guidance strategy that conditions each diffusion step with multiple granularities to improve step-wise regional attention. Furthermore, we propose learning the mutual information in each granularity by enforcing Maximum-Mean Discrepancy regularization during the diffusion forward process. We evaluate the effectiveness of our DiffMIC on three medical classification tasks with different image modalities, including placental maturity grading on ultrasound images, skin lesion classification using dermatoscopic images, and diabetic retinopathy grading using fundus images. Our experimental results demonstrate that DiffMIC outperforms state-of-the-art methods by a significant margin, indicating the universality and effectiveness of the proposed model. Our code will be publicly available at https://github.com/scott-yjyang/DiffMIC.

==> section2-relatedwork.tex <==
\section{Related Work}
\label{sec:litre}
Diffusion Probabilistic Models, which iteratively improve a given image to obtain image quality that is on par with or better than other types of generative models, have achieved state-of-the-art results in image generation and synthesis tasks~\cite{song2020score,batzolis2021conditional,dhariwal2021diffusion,singh2022high,rombach2022high}.
%
DDPM~\cite{ho2020denoising} is a generative model based on a Markov chain, which models the data distribution by simulating a diffusion process that evolves the input data towards a target distribution.
%
LDMs~\cite{esser2021taming,rombach2022high} proposed to conduct the diffusion process on a compressed latent space of lower dimensionality with cheaper computational cost, faster inference and competitive synthesis quality.
%
While Diffusion models have achieved great success in low-level vision, their potential for high-level vision has yet to be fully explored. A few pioneer works tried to adopt the diffusion model for image segmentation and object detection tasks~\cite{amit2021segdiff,wolleb2022diffusion,gu2022diffusioninst,chen2022diffusiondet}. 
%
For example, Chen \etal~\cite{chen2022diffusiondet} applied a diffusion model for object detection by denoising the random box. CARD~\cite{han2022card} adopted the diffusion process as uncertainty estimation to improve the regression performance. 
%SegDiff~\cite{amit2021segdiff} leveraged a diffusion model to calibrate the segmentation map from both the current estimate and the input image. 
%
However and despite increasing attention to perception tasks, there are no previous solutions that adopt diffusion models for medical image classification. 
%While most segmentation methods are still processed in an image-to-image fashion, image classification, a prediction problem, apparently works in a more demanding way.


